Age-optimal Scheduling over Hybrid Channels

We consider the problem of minimizing the age of information when a source can transmit status updates over two heterogeneous channels. Our work is motivated by recent developments in 5G mmWave technology, where transmissions may occur over an unreliable but fast (e.g., mmWave) channel or a slow reliable (e.g., sub-6GHz) channel. The unreliable channel is modeled as a time-correlated Gilbert-Elliot channel at a high rate when the channel is in the 'ON' state. The reliable channel provides a deterministic but lower data rate. The scheduling strategy determines the channel to be used for transmission in each time slot, aiming to minimize the time-average age of information (AoI). The optimal scheduling problem is formulated as a Markov Decision Process (MDP), which is challenging to solve because super-modularity does not hold in a part of the state space. We address this challenge and show that a multi-dimensional threshold-type scheduling policy is optimal for minimizing the age. By exploiting the structure of the MDP and analyzing the discrete-time Markov chains (DTMCs) of the threshold-type policy, we devise a low-complexity bisection algorithm to compute the optimal thresholds. We compare different scheduling policies using numerical simulations.

==> sections/abstract.tex <==
\begin{abstract}
We consider the problem of minimizing the age of information when a source can transmit status updates over two heterogeneous channels. Our work is motivated by recent developments in 5G mmWave technology, where transmissions may occur over an unreliable but fast (e.g., mmWave) channel or a slow reliable (e.g., sub-6GHz) channel. The unreliable channel is modeled as a time-correlated Gilbert-Elliot channel at a high rate when the channel is in the “ON” state. The reliable channel provides a deterministic but lower data rate. The scheduling strategy determines the channel to be used for transmission in each time slot, \textcolor{blue}{aiming} to minimize the time-average age of information (AoI). The optimal scheduling problem is formulated as a Markov Decision Process (MDP), which \textcolor{blue}{is challenging to solve} because super-modularity does not hold in a part of the state space.
We address the challenge and show that a multi-dimensional threshold-type scheduling policy is optimal for minimizing the age. By exploiting the structure of the MDP \textcolor{blue}{and analyzing the discrete time Markov chains (DTMCs) of the threshold-type policy}, a low-complexity bisection algorithm is devised to compute the optimal thresholds. %\textcolor{blue}{Our result holds for arbitrary values of the self-transition probabilities and delay}.  
Numerical simulations are provided to compare different scheduling policies. %where information can be transmitted
\end{abstract}
%Numerical simulations are provided to demonstrate the superior performance of the optimal scheduling policy. %The MDP structure based on two largely different channels with time correlation is complicated, which makes the problem challenging. 
%The difficulty of the MDP is due to its complicated time-correlation structure for two reasons: (i) the two channels have different transmission time durations and (ii) the state of the unreliable (mmWave) channel is correlated over time. 
%To solve this problem we first show that 

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}
This work was supported in part by the Army Research Office under Grant Number W911NF-21-1-0244, NSF grants: CNS-1901057, CNS- 2007231, CNS-1618520, CNS-1409336, and the Office of Naval Research under Grant N00014-17-1-241.

==> sections/bio.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/Jiayu.eps}}]{Jiayu Pan} received the B.S. degree in Physics from Shanghai Jiao Tong University, Shanghai, China in 2017. He is currently pursuing the Ph.D. degree with the Electrical and Computer Engineering Department, at the Ohio State University, OH, USA. His research interests include wireless communication and age of information. He received the First Prize Scholarship from Shanghai Jiao Tong University in 2015.    
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/Ahmed.eps}}]{Ahmed M. Bedewy} received the B.S. and M.S. degrees in electrical and electronics engineering from Alexandria University, Alexandria, Egypt, in 2011 and 2015, respectively, and the Ph.D. degree in electrical and computer engineering from The Ohio State University, OH, USA, in 2021. His research interests include wireless communication, cognitive radios, resource allocation, communication networks, information freshness, optimization, and scheduling algorithms. He received the Awarded Certificate of Merit and First Class Honors for being
one of the top ten undergraduate students, for the period 2006–2008, and the First, for the period 2008–2011, in electrical and electronics engineering. His article received the runner-up for the Best Paper Award of ACM MobiHoc 2020.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/Yin-Sun.eps}}]{Yin Sun} (S'08-M'11-SM'20) 
received the B.Eng.
and Ph.D. degrees in electronic engineering from
Tsinghua University in 2006 and 2011, respectively.
From 2011 to 2017, he was a Post-Doctoral Scholar
and a Research Associate with The Ohio State
University. He is currently an Assistant Professor
with the Department of Electrical and Computer
Engineering, Auburn University. He coauthored a
monograph \emph{Age of Information: A New Metric for
Information Freshness} (Morgan and Claypool Publishers,
2019). His research interests include age of
information, networking, robotic control, information theory, and machine
learning. He is a member of the ACM. His articles received the Best Student
Paper Award from the IEEE/IFIP WiOpt 2013, the Best Paper Award from
the IEEE/IFIP WiOpt 2019, and runner-up for the Best Paper Award of ACM
MobiHoc 2020 and the 2021 Journal of Communications and Networks (JCN)
Best Paper Award. He received the Auburn Author Award of 2020. He cofounded
the Age of Information Workshop in 2018.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/shroff.eps}}]{Ness B. Shroff} (S’91–M’93–SM’01–F’07)
received the Ph.D. degree in electrical engineering from Columbia University in 1994. 
He joined Purdue University immediately thereafter as an Assistant Professor with the School of Electrical and 
Computer Engineering.  At Purdue, he became a Full Professor of ECE and the director of a university-wide center on wireless systems and 
applications in 2004. In 2007, he joined The Ohio State University, where he holds the Ohio Eminent Scholar Endowed Chair in 
networking and communications, in the departments of ECE and CSE. He holds or has held visiting (chaired) professor positions at Tsinghua 
University, Beijing, China, Shanghai Jiaotong University, Shanghai, China, and IIT Bombay, Mumbai, India. He has received numerous best paper awards for his 
research and is listed in Thomson Reuters’ on The World’s Most Influential Scientific Minds, and is noted as a Highly Cited Researcher by Thomson Reuters. He currently serves as the steering committee chair for ACM Mobihoc and the Editor in Chief of the IEEE/ACM Transactions on Networking. He received the IEEE INFOCOM Achievement Award for seminal contributions to scheduling and resource allocation in wireless networks.  
\end{IEEEbiography}

==> sections/proof-backup.tex <==

%\section{Proof of Main Results}
\section{Appendices}
\label{mainproof}

In this section we prove our main results: Theorem \ref{theorem2} (Section \ref{proof2}) and Theorem \ref{theorem3} (Section \ref{proof3}). In Section \ref{discountedA}, we describe a discounted problem that helps to solve average problem \eqref{avg}. In Section \ref{proof2}, we introduce Proposition \ref{lemma2} which plays an important role in proving Theorem \ref{theorem2}. Section \ref{proof3} provides the proof of Theorem \ref{theorem3}. %we firstly show that the optimal policy belongs to a restricted action space where one always transmit the packet if the server is idle. Then  %Section \ref{proof3bc} provides the proof of Theorem \ref{theorem3} (b) and (c) in Section \ref{mainresults}. The difference between Section \ref{proof3} and \ref{proof3bc} is that Section \ref{proof3} utilizes similar technique with Section \ref{proof2} and shows that always choosing Channel $1$ is optimal if $(p,q,d)\in \textbf{B}_1 \cup \textbf{B}_4$, while Section \ref{proof3bc} provides the exact solution to computing optimal age and thresholds, since in general no constant policy can achieve optimality.        

\subsection{Preliminaries}\label{discountedA}





To solve Problem \eqref{avg}, we introduce a discounted problem below. The objective is to solve the discounted sum of expected cost given an initial state \textbf{s}:
\begin{equation}
J^\alpha (\textbf{s}) = \inf_{\pi\in\Pi'} \lim_{T\rightarrow \infty} \sum_{t=0}^{T} \mathbb{E}[\alpha^{t} \Delta^\pi(t)|\textbf{s}(0)=\textbf{s}], 
\label{disc}
\end{equation} where $\alpha\in (0,1)$ is the discount factor. We call $J^\alpha (\textbf{s})$ the \emph{value function} given the initial state \textbf{s}. Recall that we use \textbf{s}$=(\delta,l_1,l_2)$ to denote the system state, where $\delta$ is the age value and $l_1,l_2$ are the state of Channel $1$ and Channel $2$. From Lemma \ref{zerowait}, we only need to consider $\pi\in \Pi'$ instead of $\pi\in \Pi$. 

The value function $J^\alpha (\textbf{s})$ satisfies a following property:
%Suppose $J^\alpha (\cdot):\textbf{S}\rightarrow \mathbb{R}$ is the optimal objective value of \eqref{disc}, 
\begin{lemma}
For any given $\alpha$ and \textbf{s}, $J^\alpha(\textbf{s})<\infty$. 
\label{finite}
\end{lemma}
\begin{proof}
\ifreport
See Appendix \ref{app1}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}


A policy $\pi$ is deterministic stationary if $\pi(t)=Z(\textbf{s}(t))$ at any time $t$, where $Z: \textbf{S}\rightarrow \Pi'$ is a deterministic function. According to \cite{sennott1989average}, and Lemma \ref{finite}, there is a direct result for Problem \eqref{disc}:

\begin{lemma}
(a) The value function $J^\alpha(\textbf{s})$ satisfies the Bellman equation
\begin{equation}
\begin{split}
   Q^\alpha(\textbf{s},u) & \triangleq \delta + \alpha \sum_{\textbf{s}'\in \textbf{S}}P_{\textbf{s}\textbf{s}'}(u)J^\alpha(\textbf{s}'),\\
   J^\alpha(\textbf{s}) & = \min_{u\in \Pi'} Q^\alpha(\textbf{s},u). \end{split}
\label{discounted-lemma1}
\end{equation}

(b) There exists a deterministic stationary policy ${\mu}^{\alpha,*}$ that satisfies Bellman equation \eqref{discounted-lemma1}. The policy ${\mu}^{\alpha,*}$ solves Problem \eqref{disc} for all initial state \textbf{s}. 

(c) Assume that $J^\alpha_0(\textbf{s})=0$ for all \textbf{s}. For $n\ge 1$, $J^\alpha_n$ %$(\cdot):\textbf{S}\rightarrow \mathbb{R}$ 
is defined as %the following value iteration  
\begin{equation} \begin{split} 
   Q^\alpha_{n}(\textbf{s},u) & \triangleq  \delta +\alpha\sum_{\textbf{s}'\in\textbf{S}} P_{\textbf{s}\textbf{s}'}(u) J^\alpha_{n-1}(\textbf{s}'),\\
   J^\alpha_{n}(\textbf{s}) & = \min_{u\in \Pi'} Q^\alpha_{n}(\textbf{s},u),  \label{value-iterate} \end{split}
\end{equation}
then $\lim_{n\rightarrow \infty} J^\alpha_n(\textbf{s})=J^\alpha(\textbf{s})$ for every \textbf{s}.
\label{lemma1}
\end{lemma}


Also, since the cost function is linearly increasing in age, utilizing Lemma \ref{lemma1} (c), we also have  \begin{lemma}\label{monotonicity}
For all given $l_1$ and $l_2$, $J^\alpha (\delta,l_1,l_2)$ is increasing in $\delta$. 
\end{lemma}
\begin{proof}
\ifreport
See Appendix \ref{monotonicityapp}.
\else
See our technical report \cite{pan2020age}.
\fi
 \end{proof}


Since Problem \eqref{disc} satisfies the properties in Lemma \ref{lemma1}, utilizing Lemma \ref{lemma1} and Lemma \ref{monotonicity}, the following Lemma gives the connection between Problem \eqref{avg} and Problem \eqref{disc}. 

\begin{lemma} 
(a) There exists a stationary deterministic policy that is optimal for Problem \eqref{avg}. 

(b) There exists a value $J^*$ for all initial state $\textbf{s}$ such that    
\begin{equation*}
    \lim_{\alpha\rightarrow 1^-}(1-\alpha)J^\alpha (\textbf{s}) = J^*.
\end{equation*} 
Moreover, $J^*$ is the optimal average cost for Problem \eqref{avg}.

(c) For any sequence $(\alpha_n)_n$ of discount factors that converges to $1$, there exists a subsequence $(\beta_n)_n$ such that $\lim_{n\rightarrow \infty}{\mu}^{\beta_n,*} = {\mu^*}$. Also, ${\mu^*}$ is the optimal policy for Problem \ref{avg}. 
\label{theorem1}
\end{lemma}

\begin{proof}
\ifreport
See Appendix \ref{proof1}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}

Lemma \ref{theorem1} provides the fact that: We can solve Problem \eqref{disc} to achieve Problem \eqref{avg}. The reason is that the optimal policy of Problem \eqref{disc} converges to the optimal policy of Problem \eqref{avg} in a limiting scenario (as $\alpha\rightarrow 1$).   

%Lemma \ref{theorem1} tells there exists an optimal $\mu^*: \bm{S} \rightarrow \{0,1,2\}$.

%Note that if the state of Channel $2$ is $0$, the policy is idle. So solving $\mu^*$ is equivalent to analysing the structure of binary $\mu^*(\delta,l_1,0)$ with $\delta=1,2,...$ and $l_1 = 0,1$. 

\subsection{Proof of Theorem \ref{theorem2} }\label{proof2}

We begin with providing an optimal structural result of discounted policy $\mu^{\alpha,*}$. Then, we achieve the average optimal policy ${\mu^*}$ by letting $\alpha\rightarrow 1$.

\begin{definition}
For any discount factor $\alpha \in (0,1)$, the channel parameters $p,q\in (0,1)$ and $d\in \{2,3,...\}$, we define
\begin{equation}
\begin{split}
    \textbf{B}_1(\alpha) & =\{ (p,q,d): F(p,q,d,\alpha)\le 0, H(p,q,d,\alpha)\le 0 \}, \\     
    \textbf{B}_2(\alpha) & =\{ (p,q,d): F(p,q,d,\alpha)> 0, G(p,q,d,\alpha)\le 0 \}, \\
    \textbf{B}_3(\alpha) & =\{(p,q,d): F(p,q,d,\alpha)> 0, G(p,q,d,\alpha)> 0 \}, \\
    \textbf{B}_4(\alpha) & =\{(p,q,d): F(p,q,d,\alpha)\le 0, H(p,q,d,\alpha)> 0 \}, 
    \end{split}\end{equation}
where functions $F(\cdot),G(\cdot),H(\cdot):\Theta\times(0,1)\rightarrow \mathbb{R}$ are defined as:  \begin{equation}\begin{split}
    F(p,q,d,\alpha)&=\sum_{i=0}^{\infty} (\alpha p)^i-\sum_{i=0}^{d-1}\alpha^i, \\
    %G(p,q,d,\alpha)&=1-(1-\alpha(1-q))\sum_{i=0}^{d}\alpha^i,\\
    G(p,q,d,\alpha)&=1+\alpha(1-q)\sum_{i=0}^{d-1}\alpha^i-\sum_{i=0}^{d-1}\alpha^i,\\
    H(p,q,d,\alpha)&=1+\alpha(1-q)\sum_{i=0}^{\infty}(\alpha p)^i-\sum_{i=0}^{d-1}\alpha^i. 
    \end{split}\end{equation}%\label{def1}
\end{definition}
 Observe that all four regions $\textbf{B}_i(\alpha)$ converge to $\textbf{B}_i$ as the discount factor $\alpha\rightarrow 1$, where the regions $\textbf{B}_i$ are described in Definition \ref{def1}.  

The optimal structural result of Problem \eqref{disc} with a discount factor $\alpha$ is provided in the following proposition (Note that Theorem \ref{theorem2} can be immediately shown from Proposition \ref{lemma2}, Lemma \ref{theorem1} and the convergence of the regions $\textbf{B}_i(\alpha)$ to $\textbf{B}_i$ (for $i=1,2,3,4$) as $\alpha\rightarrow 1$):

\begin{proposition}

There exists a threshold type policy $\mu^{\alpha,*}(\delta,l_1,0)$ on age $\delta$ that is the solution to Problem \eqref{disc} such that:

(a) If $l_1 = 0$ and $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_4(\alpha)$, then $\mu^{\alpha,*}(\delta,l_1,0)$ is non-increasing in the age $\delta$. 

(b) If $l_1 = 0$ and $(p,q,d)\in \textbf{B}_2(\alpha)\cup \textbf{B}_3(\alpha)$, then $\mu^{\alpha,*}(\delta,l_1,0)$ is non-decreasing in the age $\delta$. 

(c) If $l_1 = 1$ and $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_2(\alpha)$, then $\mu^{\alpha,*}(\delta,l_1,0)$ is non-increasing in the age $\delta$. 

(d) If $l_1 = 1$ and $(p,q,d)\in \textbf{B}_3(\alpha)\cup \textbf{B}_4(\alpha)$, then $\mu^{\alpha,*}(\delta,l_1,0)$ is non-decreasing in the age $\delta$. 
%There exists a threshold type policy $\mu^\alpha(\delta,l_1,0)$ on age $\delta$ that is the solution to Problem \eqref{disc}. The detailed structure type is as follows in (a) and (b):

%(a) The policy $\mu^\alpha(\delta,0,0)$ is non-increasing in $\delta$ if $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_4(\alpha)$, non-decreasing if $(p,q,d)\in \textbf{B}_2(\alpha)\cup \textbf{B}_3(\alpha)$.

%(b) The policy $\mu^\alpha(\delta,1,0)$ is non-increasing in $\delta$ if $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_2(\alpha)$, non-decreasing if $(p,q,d)\in \textbf{B}_3(\alpha)\cup \textbf{B}_4(\alpha)$.
\label{lemma2}
\end{proposition}

%\begin{proof}
% Please see Section \ref{proof2} for details. 
%\end{proof} 

%So Theorem \ref{theorem2} can be immediately shown from Proposition \ref{lemma2}, Lemma \ref{theorem1} and the convergence of the regions $\textbf{B}_i(\alpha)$ to $\textbf{B}_i$ (for $i=1,2,3,4$) as $\alpha\rightarrow 1$. Thus, the remainder of Section \ref{proof2} provides the main proof of Proposition \ref{lemma2}. This is the start of the proof of Proposition \ref{lemma2}. 




%In the remaining sections, for ease of description, we omit the subscription $\alpha$ in $J^\alpha (\cdot)$, $J^\alpha_n (\cdot)$, $Q^\alpha (\cdot)$, $Q^\alpha_n (\cdot)$, $\mu^\alpha (\cdot)$ and $\mu^\alpha_n (\cdot)$.

Since Channel $1$ and Channel $2$ have different delays, we are not able to show that the optimal policy is threshold type by directly observing the Bellman equation like \cite{altman2019forever}. Thus, we will use the concept of \emph{supermodularity} \cite[Theorem 2.8.2]{topkis1998supermodularity}. The domain of age set and decision set in the Q-function is $\{1,2,...\}\times \{1,2\}$, which is a \emph{lattice}. Given a positive $s$, the subset $\{s,s+1,...\}\times \{1,2\}$ is a \emph{sublattice} of $\{1,2,...\}\times \{1,2\}$. Thus, if the following holds for all $\delta>s$: 
\begin{equation}\begin{split}
& Q^\alpha (\delta,l_1,0,1)-Q^\alpha(\delta-1,l_1,0,1) \\ \le  & Q^\alpha(\delta,l_1,0,2)-Q^\alpha(\delta-1,l_1,0,2), \end{split} \label{modular}  
\end{equation}
then the Q-function $Q^\alpha(\delta,l_1,0,u)$ is supermodular in $(\delta,u)$ for $\delta>s$, which means the optimal decision \begin{equation}
    \mu^{\alpha,*}(\delta,l_1,0) =\mathrm{argmin}_{u}Q^\alpha(\delta,l_1,0,u)
\end{equation} is non-increasing in $\delta$ for $\delta\ge s$. If the inequality of \eqref{modular} is inversed, then we call $Q^\alpha(\delta,l_1,0)$ is submodular in $(\delta,u)$ for  $\delta>s$, and $\mu^{\alpha,*}(\delta,l_1,0)$ is non-decreasing in $\delta$ for $\delta\ge s$. 



%(\text{or}\le)

For ease of notations, we give Definition \ref{def2}:

\begin{definition} Given $l_1\in \{0,1\}$, $u\in \{1,2\}$, %$n\ge 0$ 
\begin{equation}
L^\alpha(\delta,l_1,u)\triangleq Q^\alpha(\delta,l_1,0,u)-Q^\alpha(\delta-1,l_1,0,u).
\end{equation}  
\label{def2}
\end{definition} \vspace{-8pt} %L_n(\delta,l_1,u)\triangleq Q_n(\delta,l_1,0,u)-Q_n(\delta-1,l_1,0,u)
Note that $L^\alpha(\delta,l_1,1)$ is the left hand side of \eqref{modular}, and $L^\alpha(\delta,l_1,2)$ is the right hand side of \eqref{modular}. %Also, $L(\delta,l_1,u)$ is also called the age difference function under the action $u$. Thus, the Q-function $Q(\delta,l_1,0,u)$ is supermodluar (or submodular) in $(\delta,u)$ for $\delta>s$, if $L(\delta,l_1,1)\le($or$ \ge) L(\delta,l_1,2)$ for $\delta>s$. 

However, because of the mismatch of delays in our problem, most of the well-known techniques to show supermodularity (e.g., \cite{puterman1990markov},\cite{ngo2009optimality},\cite{krishnamurthy2016partially} etc) do not apply in our setting. Thus, we need a new approach to show the supermodularity. Our key idea is as follows: First, we show that $L^\alpha(\delta,l_1,2)$ is a constant (see Lemma \ref{g2m} below), then we compare $L^\alpha(\delta,l_1,1)$ with the constant (see the proofs of Lemma \ref{l0m} and Lemma \ref{l1m} below).
 %The right hand side $L(\delta,l_1,2)$ has the following nice property, which is a constant:
 
Suppose that $m\triangleq \sum_{i=0}^{d-1} \alpha^i$, and we have:
 \begin{lemma}\label{g2m}
 For all $\delta\ge 2$ and $l_1\in \{0,1 \}$, $L^\alpha(\delta,l_1,2)=m$. 
% \begin{equation}\begin{split}
%   L(\delta,l_1,2)= m.\end{split}
% \end{equation}
 \end{lemma}
 
 \begin{proof}
 \ifreport
See Appendix \ref{g2mapp}.
\else
See our technical report \cite{pan2020age}.
\fi
 \end{proof}
% Lemma \ref{g2m} tells us that the right hand side function $L(\delta,l_1,2)$, is the discounted sum of constant $1$ and the length is the delay of Channel $2$. %Note that Lemma \ref{g2m} only holds if the cost function is linear in age $\delta$.
 
%In the following sections we may use $m$ or $\sum_{i=0}^{d} \alpha^i$ interchangeably.
%Remember that $F(p,q,d,\alpha)=\sum_{i=0}^{\infty} (\alpha p)^i-m$. 
%From Lemma \ref{g2m}, judging $L(\delta,l_1,1)\le( \text{or} \ge) L(\delta,l_1,2)$ turns into whether $L(\delta,l_1,1)\le (\text{or}\ge)$  $m$.

%Also, the constant $m$ has the following property: 

%Thus, benefiting from Lemma \ref{g2m}, we next show the relation between $L(\delta,0,1)$ and the constant $m$.
Also, we have
\begin{lemma}\label{l0m}
(a) If $l_1=0$ and $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_4(\alpha)$, then $Q^\alpha(\delta,l_1,0,u)$ is supermodular in $(\delta,u)$ for $\delta\ge 2$.

(b) If $l_1=0$ and $(p,q,d)\in \textbf{B}_2(\alpha)\cup \textbf{B}_3(\alpha)$, then $Q^\alpha(\delta,l_1,0,u)$ is submodular in $(\delta,u)$ for $\delta\ge 2$.
\end{lemma}

\begin{proof}
\ifreport
See Appendix \ref{l0mapp}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}

%From Lemma \ref{g2m} and Lemma \ref{l0m}, we directly find that $L(\delta,0,1)\le L(\delta,0,2)$ if the system parameters $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_4(\alpha)$. Also, $L(\delta,0,1)> L(\delta,0,2)$ if the system parameters $(p,q,d)\in \textbf{B}_2(\alpha)\cup \textbf{B}_3(\alpha)$.   
%Thus, the Q-function $Q(\delta,0,0,u)$ is supermodular in $(\delta,u)$ and

Lemma \ref{l0m} (a) implies that $\mu^{\alpha,*}(\delta,0,0)$ is non-increasing in $\delta$ if $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_4(\alpha)$. Lemma \ref{l0m} (b) implies that $\mu^{\alpha,*}(\delta,0,0)$ is non-increasing in $\delta$ if $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_4(\alpha)$.
%Also, the Q-function $Q(\delta,0,0,u)$ is submodular in $(\delta,u)$ and $\mu(\delta,0,0)$ is non-decreasing threshold type if the system parameters $(p,q,d)\in \textbf{B}_2(\alpha)\cup \textbf{B}_3(\alpha)$.  
Thus, Proposition \ref{lemma2} (a) and (b) hold.  

Lemma \ref{l0m} gives the result when the state of Channel $1$ is $0$. We then need to solve when the state of Channel $1$ is $1$. Different from $Q^\alpha(\delta,0,0,u)$, the Q-function $Q^\alpha(\delta,1,0,u)$ does not satisfy supermodular (or submodular) in ($\delta,u$) for all the age value. Thus, we give a weakened condition: we can find out a value $s$, such that the Q-function $Q^\alpha(\delta,1,0,u)$ is supermodular (or submodular) for a partial set $s,s+1,...$ and $\mu^{\alpha,*}(\delta,1,0)$ is a constant on the set $1,2,...,s$. Then, $\mu^{\alpha,*}(\delta,1,0)$ is non-increasing (or non-decreasing).      

Thus, to solve Proposition \ref{lemma2} (c) and (d), we provide the following lemma:   
%Thus, according to \eqref{A10} and \eqref{A1022}, the focus is comparing $J(\delta+1,0,0)-J(\delta,0,0)$ with $m$.
%We firstly provide a Lemma: 

%Lemma \ref{11d110} helps for introducing a property for optimality of switch type policy: 

%Now we start proving (b)

%Lemma \ref{lemma-switch} is useful for solving the following lemma which is the sufficient condition for theorem \ref{lemma2} (b):

\begin{lemma}\label{l1m}
(a) If $l_1=1$ and $(p,q,d)\in \textbf{B}_1(\alpha)\cup \textbf{B}_2(\alpha)$, 
then there exists a positive integer $s$, such that $Q^\alpha(\delta,l_1,0,u)$ is supermodular in $(\delta,u)$ for $\delta > s$, and $\mu^{\alpha,*}(\delta,l_1,0)$ is always $1$ or always $2$ for all $\delta \le s$. %Thus, $\mu(\delta,1,0)$ is nonincreasing.  

(b) If $l_1=1$ and $(p,q,d)\in \textbf{B}_3(\alpha)\cup  \textbf{B}_4(\alpha)$, then there exists a positive integer $s$, such that $Q^\alpha(\delta,l_1,0,u)$ is submodular in $(\delta,u)$ for $\delta > s$, and $\mu^{\alpha,*}(\delta,l_1,0)$ is always $1$ or always $2$ for all $\delta \le s$.

%either of the two cases holds: ($1$) The policy $\mu(\delta,1,0)$ is always $1$ or always $2$. ($2$) there exists a positive integer $s$, such that the left hand side $L(\delta,1,1) > m$ for all $\delta > s$ and $\mu(\delta,1,0)$ is always $1$ or always $2$ for all $\delta \le s$.

%Thus, $\mu(1,1,0)$ is nondecreasing. 

%(c) If $(p,q,d)\in \textbf{B}_2(\alpha)$, then there exists $s\ge 0$, such that $L(\delta,1,1) \le L(\delta,1,2)$ for all $\delta > s$ and $\mu(\delta,1,0)=1$ for all $\delta \le s$. Thus $\mu(1,1,0)$ is nonincreasing. 

%(d) If $(p,q,d)\in \textbf{B}_3(\alpha)$, then there exists $s\ge 0$, such that $L(\delta,1,1) > L(\delta,1,2)$ for all $\delta > s$ and $\mu(\delta,1,0)=1$ for all $\delta \le s$. Thus $\mu(1,1,0)$ is nondecreasing. 
\end{lemma}

\begin{proof}
\ifreport
See Appendix \ref{l1mapp}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}

%There is one difference between Lemma \ref{l1m} and Lemma \ref{l0m}. Lemma \ref{l1m} does not provide a strong result e.g., the left hand side $L(\delta,1,1)\le$ or $>m$ for all the age $\delta>1$. Compared with $L(\delta,0,1)$, the left hand side $L(\delta,1,1)$ may not satisfy this condition. For example, take the system parameters $(p,q,d)=(0.8,0.3,2)$ and the discounted factor $\alpha=0.9$. Despite $\mu(\delta,1,0)=1$ is constant on age $\delta$, the difference $L(\delta,1,1)-m$ is not all positive on age $\delta$. However, Lemma \ref{l1m} is sufficient to show the policy $\mu(\delta,1,0)$ is threshold type.  

% We look at the two cases in Lemma \ref{l1m} (a). In case ($1$), the constant policy is a non-increasing policy. In case ($2$), 
 
% Lemma \ref{g2m} implies that the right hand side $L(\delta,1,2)=m$ for all $\delta$. Thus, in Lemma \ref{l1m}, we get $L(\delta,1,1)\le L(\delta,1,2)$ for age $\delta>s$. 
 
 Lemma \ref{l1m} (a) implies that  $\mu^{\alpha,*}(\delta,1,0)$ is non-increasing for $\delta\ge s$ and is constant for for $\delta\le s$. Thus, $\mu^{\alpha,*}(\delta,1,0)$ is non-increasing in $\delta$. Similarly, Lemma \ref{l1m} (b) implies that $\mu^{\alpha,*}(\delta,1,0)$ is non-decreasing for $\delta>0$. Thus, we have shown Proposition \ref{lemma2} (c) and (d).  

 Overall, Lemma \ref{g2m} and Lemma \ref{l0m} shows Proposition \ref{lemma2} (a) and (b). Lemma \ref{g2m} and Lemma \ref{l1m} shows Proposition \ref{lemma2} (c) and (d). Thus we have completed the proof of Proposition \ref{lemma2}.
 
 Finally, Proposition \ref{lemma2}, Lemma \ref{theorem1} and the convergence of  $\textbf{B}_1(\alpha),...\\ \textbf{B}_4(\alpha)$ to $\textbf{B}_1,...,\textbf{B}_4$ show Theorem \ref{theorem2}. 
\subsection{Proof of Theorem \ref{theorem3}}\label{proof3}

For $(p,q,d)\in \textbf{B}_1$, we firstly prove that $\mu^*(\delta,0,0)=1$ and then show $\mu^*(\delta,1,0)=1$.  

\begin{lemma}\label{mu00in1and4}
If $(p,q,d)\in \textbf{B}_1 \cup \textbf{B}_4$, then the optimal decisions at states $(\delta,0,0)$ for all $\delta$ are $1$.
\end{lemma}

\begin{proof}
\ifreport
See Appendix \ref{mu00in1and4app}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}

On the other hand, when $l_1=1$, we have the following:

\begin{lemma}\label{mu110for1}
If $(p,q,d)\in \textbf{B}_1 $, then the optimal decision $\mu^*(1,1,0)=1$. 
\end{lemma}
\begin{proof}
\ifreport
See Appendix \ref{mu110for1app}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}

Since $\mu^*(\delta,1,0)$ is non-increasing in the region $\textbf{B}_1$ by Theorem \ref{theorem2}, Lemma \ref{mu110for1} implies that $\mu^*(\delta,1,0)=1$ for all $\delta$.
 Thus Theorem \ref{theorem3} (a) follows directly from Lemma \ref{mu00in1and4}, Lemma \ref{mu110for1}. % and Lemma \ref{theorem1}. 
 
%Before we further move to the other regions $\textbf{B}_2,\textbf{B}_3,\textbf{B}_4$, we need to emphasize that the optimal decision $\mu^*(1,1,0)$ and $\mu^*(d,1,0)$ is \emph{sufficient} for the optimal decision set $\mu^*(\delta,1,0)$ with $\delta\ge1$. This is because any binary policy cannot reach the states $(2,1,0),...,(d-1,1,0)$,$(d+1,1,0)$,... In addition, 
While the result of case $(p,q,d)\in \textbf{B}_1$ is simple to describe, the result of cases $(p,q,d)\in \textbf{B}_2$, $\textbf{B}_3$ and $\textbf{B}_4$ are not.   
For other cases $(p,q,d)\in \textbf{B}_2$, $\textbf{B}_3$ and $\textbf{B}_4$, since the optimal decision may not be constant, we give an exact solution based on solving corresponding Markov Chains. 
Since Channel $1$ is Markovian, there are two non-symmetric states $(\delta,1,0),(\delta,0,0)$ for the same age $\delta$. 
This complicates the problem: the Markov chain varies based on the restarting states $(1,1,0)$, $(d,1,0)$ and $(d,0,0)$. %This is because any given state may be recurrent in one scenario (the decisions of restarting states) but transient in other scenario. 
Therefore, we need to enumerate all the feasible cases based on the decisions $(1,1,0)$, $(d,1,0)$ and and $(d,0,0)$. However, some of the Markov Chain types (out of $2^3$ types) are negligible; the reasons are two folds: (1) the monotonicity is known by Theorem \ref{theorem2}, and (2) the following lemma:

\begin{lemma}\label{lemma-switch-avg}
If Channel $1$ is positive-correlated, i.e., $p+q\ge 1$, and $\mu^{*}(\delta,0,0)=1$, then $\mu^{*}(\delta,1,0)=1$.
Conversely, if Channel $1$ is negative-correlated, i.e. $p+q\le 1$, and $\mu^{*}(\delta,0,0)=2$, then $\mu^{*}(\delta,1,0)=2$.
\end{lemma}
\begin{proof}
See 
\ifreport
Appendix \ref{lemma-switchapp}.
\else
our technical report \cite{pan2020age}.
\fi
\end{proof}


%are feasible according to 
%\ifreport
%Lemma \ref{lemma-switch} in Appendix %\ref{l1mapp}.
%\else
%our technical report \cite{pan2020age}.
%\fi
 Note that the decision at $(d,0,0)$ is equivalent to whether the threshold of $\mu^*(\delta,0,0)$ is larger or smaller than $d$. Thus, we use $s$ to denote the threshold of $\mu^*(\delta,0,0)$.

%Thus, $u(1,1,0)=1$ is sufficient to show the optimal policy is always choosing Channel $1$. And the optimal non-decreasing threshold $\lambda_1^*\in \{ 2,3,...\}$. Thus, we provide the following lemma:  

%\begin{lemma}\label{mu110for4}
%If $(p,q,d)\in \textbf{B}_4 $, then the policy $\mu(1,1,0)=1$ 
%\end{lemma}
%\begin{proof} Please see Appendix \ref{mu110for4app} for details. 

%\end{proof}
  

%\subsection{Proof of Theorem \ref{theorem3} (b) and (c)}\label{proof3bc}

 For $(p,q,d)\in \textbf{B}_2 $, $\mu^*(\delta,1,0)$ is non-increasing, and $\mu^*(\delta,0,0)$ is non-decreasing. Note that $(p,q,d)\in \textbf{B}_2 $ implies $p+q\ge 1$.
 
 According to Lemma \ref{lemma-switch-avg}, if $\mu^*(1,1,0)=2$, then $\mu^*(1,0,0)=2$, hence $\mu^*(\delta,0,0)=2$ for all $\delta$. Thus, there are two possible types of Markov Chains regarding $\mu^*(d,1,0)=1$ or $\mu^*(d,1,0)=2$.
  If $\mu^*(1,1,0)=1$, then $\mu^*(\delta,1,0)=1$ for all $\delta$, there are two possible types of Markov Chains regarding the threshold $s>d$ or $s\le d$.  
 
 %In Section \ref{C}, we have discussed that the Markov chain varies based on the restarting states $(1,1,0)$, $(d,1,0)$, and $(d,0,0)$. Thus, we conclude that
 Thus, for $(p,q,d)\in \textbf{B}_2 $, there are four possible ways to represent the Markov Chain diagram of the threshold policy based on the value of the threshold $s$ and the optimal decision at states $(d,l_1,0)$ and $(1,1,0)$.
 
 \ifreport
 
 
 \else
For $(p,q,d)\in \textbf{B}_3 $ and $\textbf{B}_4$, the technical analysis is similar with the previous case when $(p,q,d)\in \textbf{B}_2$.

In conclusion, for $(p,q,d)\in \textbf{B}_2$, $ \textbf{B}_3$ or $\textbf{B}_4$, the problem turns into a couple of minimization of average age over the possible threshold values. The optimal age is the minimum of the derived ages and the optimal thresholds are based on the case with the minimum. This proves Theorem \ref{theorem3}. Due to the space limit, please see our technical report \cite{pan2020age} for the complete description of Section \ref{proof3} 
 
 \fi
 
  (see
 \ifreport
Appendix \ref{markovapp}
\else
our technical report \cite{pan2020age}
\fi
for the corresponding Markov Chains and derivations): 
\begin{itemize}
    \item 
 The threshold $s>d$. The optimal decisions $\mu^*(1,1,0)=\mu^*(d,1,0)=1$ ($\lambda^*_1=1$). Then average age is derived as $f_{1}(s)/g_{1}(s)$. The functions $f_{1}(s),g_{1}(s)$ are described in 
 \ifreport
Table \ref{fg}.
\else
our technical report \cite{pan2020age}.
\fi
Note that $\beta_1$ described in Definition \ref{defthm} originates from minimizing $f_1(s)/g_1(s)$. 
  \item 
 The threshold $s\le d$, and the optimal decisions $\mu^*(1,1,0)=\mu^*(d,1,0)=1$ ($\lambda^*_1=1$). Then the average age is $f_{2}(s)/g_{2}(s)$. The functions $f_{2}(s),g_{2}(s)$ are described in 
 \ifreport
Table \ref{fg}.
\else
our technical report \cite{pan2020age}.
\fi
Note that $\beta_2$ described in Definition \ref{defthm} originates from minimizing $f_2(s)/g_2(s)$.
  \item 
 The threshold $s=1$, and the optimal decisions $\mu^*(1,1,0)=2, \mu^*(d,1,0)=1$ ($\lambda^*_1=1\in \{2,3,...,d\}$). %The markov chain is described in
% \ifreport
% Appendix \ref{markov3app}.
% \else
% our technical report \cite{pan2020age}.
 %\fi
 The average age is a constant $f_0/g_0$ and is described in 
 \ifreport
Table \ref{fg}.
\else
Table \ref{fg-conference}.
\fi
  \item 
 The threshold $s=1$. The optimal decisions $\mu^*(1,1,0)=\mu^*(d,1,0)=2$ ($\lambda^*_1\in \{d+1,d+2,...\}$). This policy means we always choose Channel $2$. So the average age is $(3/2) d-1/2$.
\end{itemize}  
% Recall that $(p,q,d)\in \textbf{B}_2$ implies the Channel $1$ is positive-correlated, i.e., $p+q\ge 1$. Thus, from 
% \ifreport
% Lemma \ref{lemma-switch} in Appendix \ref{l1mapp},
%\else
%Lemma 16 in 
%our technical report \cite{pan2020age},
%\fi
% if $\mu^*(1,1,0)=2$, then $\mu^*(1,0,0)=2$. Since $\mu^*(\delta,0,0)$ is non-decreasing in age $\delta$, so $\mu^*(\delta,0,0)=2$.

 For $(p,q,d)\in \textbf{B}_3 $ 
\ifreport
 , $\mu^*(\delta,0,0)$ and $\mu^*(\delta,1,0)$ are non-decreasing. Since $(p,q,d)\in \textbf{B}_3 $ does not imply $p+q\le 1$ or $p+q\ge 1$, we will enumerate all of the five possible ways to represent the Markov Chain diagram of the threshold policy based on the value of the threshold $s$ and the optimal decision at states $(d,l_1,0)$ and $(1,1,0)$ (see 
  \ifreport
Appendix \ref{markovapp}
\else
our technical report \cite{pan2020age}
\fi
 for the corresponding Markov Chains): 
\begin{itemize}
    \item 
 The threshold $s>d$ and the optimal decisions $\mu^*(1,1,0)=\mu^*(d,1,0)=1$ ($\lambda^*_1\in \{d+1,d+2,...\}$). The average age is derived as $f_{1}(s)/g_{1}(s)$.
   \item 
  The threshold $s>d$ and the optimal decisions $\mu^*(1,1,0)=1, \mu^*(d,1,0)=2$ ($\lambda^*_1\in \{2,...,d\}$). Then, the average age is $f_{3}(s)/g_{3}(s)$ which is described in 
   \ifreport
Table \ref{fg}.
\else
our technical report \cite{pan2020age}.
\fi
   \item 
 The threshold $s>d$ and the optimal decisions $\mu^*(1,1,0)= \mu^*(d,1,0)=2$ ($\lambda^*_1\in \{2,...,d\}$) with average age $f_{4}(s)/g_{4}(s)$ which is described in  \ifreport
Table \ref{fg}.
\else
our technical report \cite{pan2020age}.
\fi
   \item 
  The threshold $s\le d$ and the optimal decisions $\mu^*(1,1,0)=\mu^*(d,1,0)=1$ ($\lambda^*_1\in \{d+1,d+2,...\}$), with average age $f_{2}(s)/g_{2}(s)$.
   \item 
  The threshold  $s\le d$ and the optimal decision $\mu^*(d,1,0)=2$. Then regardless of $ \mu^*(1,1,0)$ ($\lambda^*_1\in \{1,2,...,d\}$), the Markov Chain is same with always choosing $2$, with average age $(3/2)d-1/2$. 
\end{itemize} 




For $(p,q,d)\in \textbf{B}_4 $, $\mu^*(\delta,1,0) $ is non-decreasing in $\delta$ from Theorem \ref{theorem2}. Also, $\mu^*(\delta,0,0)=1$ by Lemma \ref{mu00in1and4}.

If $\mu^*(1,1,0)=1$, the policy becomes always choosing Channel $1$ (since $(d,1,0)$ is transient to the Markov Chain). If $\mu^*(1,1,0)=2$, then $\mu^*(\delta,1,0)=2$ for all $\delta$.   
%from 
%\ifreport
%Appendix \ref{markovapp},
%\else
%our technical report \cite{pan2020age},
%\fi
%$f_0'/g_0'$ is the derived average age.

%This is because the states $(\delta,1,0)$ with $\delta=2,3,...$ become "transient" and will not return back to themselves.  
%From Remark \ref{remark1}, the decision $\mu^*(\delta,1,0)$ with $\delta=2,...,d-1,d+1,...$ does not affect Problem \ref{avg}. Also, the remaining state $(d,1,0)$ ends up stopping in the states $(1,1,0),(2,0,0),...$ under the policy $\mu^*(\delta,0,0)=\mu^*(1,1,0)=1$ for all the age $\delta$.
Thus, the solution of $(p,q,d)\in \textbf{B}_4 $ are two possible cases which directly gives Theorem \ref{theorem3} (d): \begin{itemize}
    \item The optimal decision $\mu^*(\delta,0,0)=1$ and $\mu^*(1,1,0)=1$. Then, the optimal policy is always choosing Channel $1$. The average age of always choosing Channel $1$ is $((1-q)(2-p)+(1-p)^2)/((2-q-p)(1-p))$ as in \eqref{always1}.
    \item The optimal decision $\mu^*(\delta,0,0)=1$ and  $\mu^*(\delta,1,0)=2$ for all $\delta$. Please see
     \ifreport
Appendix \ref{markovapp}
\else
our technical report \cite{pan2020age}
\fi
   for the corresponding Markov chain. The average age is $f'_0/g'_0$ that is described in
   \ifreport
Table \ref{fg}.   
   \else
   Table \ref{fg-conference}.
   \fi
\end{itemize}

\else
 or $\textbf{B}_4$, the technical analysis is similar with the previous case when $(p,q,d)\in \textbf{B}_2$.
 Due to the space limit, please see our technical report \cite{pan2020age} for the details. 
\fi

From our analysis in Section \ref{proof3}, we have the following conclusion: (i) If $(p,q,d)\in \textbf{B}_1$, the optimal decision is always choosing Channel $1$; 
(ii) For $(p,q,d)\in \textbf{B}_2$, $ \textbf{B}_3$ or $\textbf{B}_4$, the problem turns into a couple of minimization of average age over the possible threshold values. The optimal age is the minimum of the derived ages and the optimal thresholds are based on the case with the minimum. Thus, we have the following proposition coupled with a definition:

\begin{definition}\label{def6}
%Suppose that $i\in \{1,2,3,4 \}$. Then the sets 
%$N(i)$ are defined as: 
%$N(1)=N(3)=N(4)=\{s: s>d\}$, and $N(2)=\{s: 1\le s\le d\}$.
We denote $\beta'_1 \ldots \beta'_4$ as:
\begin{align}\beta'_{i}& =%\min_{s\in N(i)}\frac{f_{i}(s)}{g_{i}(s)}.
\min_{s\in \{ d+1,...\} }\frac{f_{i}(s)}{g_{i}(s)}, \ i\in \{1,3,4\}, \\
\beta'_{2}&=
\min_{s\in \{1,...d\} }\frac{f_{2}(s)}{g_{2}(s)}.
\label{algr}\end{align}
%Suppose that $N_a=\{1,2\}$ and $N_b=\{ 1,2,3,4\}$.
\end{definition}  

\begin{proposition}\label{theoremmin}
%Suppose $\bar{\Delta}_{\text{opt}}$ is the optimal average age of Problem \eqref{avg}. 

(a) If $(p,q,d)\in \textbf{B}_1$, 
\begin{equation}
 \bar{\Delta}_{\text{opt}}=  \frac{(1-q)(2-p)+(1-p)^2}{(2-q-p)(1-p)} .
\end{equation}

(b) If $(p,q,d)\in \textbf{B}_2$,
\begin{equation} \label{minb2}
   \bar{\Delta}_{\text{opt}} =  \min \left\{ \beta'_1,\beta'_2,\frac{f_0}{g_0},\frac{3}{2}d-\frac{1}{2}  \right\}.
\end{equation} %where $[x]_{y,z}\triangleq\min \{x,y,z\}$.

(c) If $(p,q,d)\in \textbf{B}_3$, 
\begin{equation}\label{minb3}
 \bar{\Delta}_{\text{opt}}= \min \left\{ \beta'_1,\beta'_2, \beta'_3,\beta'_4, \frac{3}{2}d-\frac{1}{2}  \right\}.
   %\bar{\Delta}_{\text{opt}} =  \Big{[}   \min_{i\in N_b} \left\{ \min_{s\in N(i)}\frac{f_{i}(s)}{g_{i}(s)} \right\} \Big{]}_{\frac{3}{2}d-\frac{1}{2}},
\end{equation} 

(d) If $(p,q,d)\in \textbf{B}_4$, 
\begin{equation}
 \bar{\Delta}_{\text{opt}}= \min \left\{ \frac{(1-q)(2-p)+(1-p)^2}{(2-q-p)(1-p)}, \frac{f'_0}{g'_0}  \right\}.
\end{equation}
\end{proposition}


Note that Proposition \ref{theoremmin} (a) comes from Lemma \ref{mu00in1and4} and Lemma \ref{mu110for1}. Proposition \ref{theoremmin} (a) directly proves Theorem \ref{theorem3} (a). Also,
Proposition \ref{theoremmin} (d) 
shows Theorem \ref{theorem3} (d). 
%and the two listed descriptions for $(p,q,d)\in \textbf{B}_4$ in this section.
%\begin{remark}
%From Proposition \ref{theoremmin}, note that $N_a$ or $N_b$ have only few elements. Thus the major computing comes from the fractional minimization i.e., $f_{i}(s)/g_{i}(s)$ over all possible thresholds $s$, in which we need to improve further.  
%\end{remark}

\ifreport
To pursue faster computation on minimization in \eqref{algr}, we introduce the following lemma: 

\begin{lemma}\label{fractional} Suppose that $i\in \{1,2,3,4 \}$.
%If $(p,q,d)\in \textbf{B}_2\cup \textbf{B}_3$, suppose that \begin{equation}\beta'_{i}=\min_{s\in N(i)}\frac{f_{i}(s)}{g_{i}(s)}. \label{algr}\end{equation}
Define
\begin{equation}h'_{i}(c)=\min_{s\in N(i)} f_{i}(s)-cg_{i}(s).\label{inlayer}\end{equation}
then for all $i=1,2,3,4$, $h'_{i}(c)\lesseqqgtr 0$ if and only if $c\gtreqqless \beta'_{i}$.  
\end{lemma}
\begin{proof} 
     \ifreport
See Appendix \ref{fractionalapp}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}
The solution of $h'_{i}(c)$ in Lemma \ref{fractional} is shown in the following lemma:

\begin{lemma}\label{fracsolution} Suppose that $i\in \{1,2,3,4 \}$.
If $(p,q,d)\in \textbf{B}_2\cup \textbf{B}_3$, then the threshold $s_{i}(c)$ defined in \eqref{threshold1} is the solution to \eqref{inlayer}, i.e., $h_i(c)=h'_i(c)$.  
\end{lemma}
\begin{proof}
     \ifreport
See Appendix \ref{app2}.
\else
See our technical report \cite{pan2020age}.
\fi
\end{proof}

From Lemma \ref{fractional}, $h_{i}(c)=0$ is the solution of \eqref{algr}. So from Lemma \ref{fracsolution}, we can immediately conclude that  
\else
From %Lemma 12 and Lemma 13 in 
our technical report \cite{pan2020age}, we get that
\fi 
for all $i\in \{1,2,3,4\}$:
\begin{equation}\label{final}
%    \beta_{i}=\min_{s\in N(i)}\frac{f_{i}(s)}{g_{i}(s)}.
\beta'_{i}=\beta_i,
\end{equation} where $\beta'_i$ is defined in Definition \ref{def6} and $\beta_{i}$ is derived in Definition \ref{defthm} with low complexity algorithm. 

Thus, Theorem \ref{theorem3} (b) and (c) are shown by \eqref{final}, Proposition \ref{theoremmin} (b) and (c) which come from the number of listed descriptions for $(p,q,d)\in \textbf{B}_2$  in this section and $(p,q,d)\in \textbf{B}_3$ in our technical report \cite{pan2020age}. Thus, we have completed the proof of Theorem \ref{theorem3}. 










\iffalse

Suppose that $\mu(d+1,1,0)=2$, then $\mu(1,1,0)=\mu(\delta,0,0)=2$ from Lemma \ref{lemma-switch}. From \eqref{switchtype1},  
\begin{equation}
\begin{split}
   & Q(1,1,0,2)-Q(1,1,0,1)\\ 
    \ge & \alpha (1-q) \Big{(} J(2,0,d)-J(2,0,0) \Big{)}\\
    + & \alpha q \Big{(} \sum_{i=0}^{d-1}\alpha^i + d\Big{(} J(d+1,0,0)-J(d+1,0,1) \Big{)} \\ +& e \Big{(} J(d+1,1,0)-J(d+1,1,1) \Big{)}  \Big{)}.
\end{split}    
\end{equation}

From round-robin property of $\mu(\delta,1,0)=\mu(\delta,0,0)=0$, $J(d+1,0,0)-J(d+1,0,1)\ge 0$, and $J(d+1,1,0)-J(d+1,1,1)\ge 0$, also, $J(2,0,d)-J(2,0,0)\ge -\alpha^d$. So 
\begin{equation*}
\begin{split}
   & Q(1,1,0,2)-Q(1,1,0,1)\\ 
    \ge & -\alpha (1-q) \alpha^d
    +  \alpha q \sum_{i=0}^{d-1}\alpha^i
    = \alpha q\times  m -\alpha^{d+1} \\ \ge & 1-(2-\alpha)m-\alpha^{d+1}=\alpha^d-\alpha^{d+1}>0.
\end{split}    
\end{equation*} which is contradictory. 

So Problem \eqref{avg} becomes only a few times of minimizing problems. The optimal thresholds of $(\delta,0,0)$, $(\delta,1,0)$ depend on which minimization problem is smallest, and $\lambda_0$ takes the optimal $s$ of that, and $\lambda_1$ is the corresponding two value based optimal decision ($\mu(1,1,0)$ and $\mu(d+1,1,0)$).    

\fi


